Mobile App Tasks with Iterative Feedback (MoTIF): Addressing Task Feasibility in Interactive Visual Environments

In recent years, vision-language research has shifted to study tasks which require more complex reasoning, such as interactive question answering, visual common sense reasoning, and question-answer plausibility prediction. However, the datasets used for these problems fail to capture the complexity of real inputs and multimodal environments, such as ambiguous natural language requests and diverse digital domains. We introduce Mobile app Tasks with Iterative Feedback (MoTIF), a dataset with natural language commands for the greatest number of interactive environments to date. MoTIF is the first to contain natural language requests for interactive environments that are not satisfiable, and we obtain follow-up questions on this subset to enable research on task uncertainty resolution. We perform initial feasibility classification experiments and only reach an F1 score of 37.3, verifying the need for richer vision-language representations and improved architectures to reason about task feasibility.

==> experiments2.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{0.9}
\setlength{\tabcolsep}{3.5pt}
    \centering
    \begin{tabular}{|l|c|c|c|}
    \hline
            %\multicolumn{2}{|l|}{Features}&  \multicolumn{3}{c|}{t = 1} & \multicolumn{3}{c|}{t = 3} & \multicolumn{3}{c|}{t = 20} \\
            %        \cline{3-11}
       Features% & First & Mid & Last & Cat & Avg & LSTM 
       & Cat & Avg & LSTM \\
        % \cline{2-19}
       % Features & \multicolumn{9}{c|}{Accuracy}  \\
       \hline
      % \textbf{(a)} & T-A & 8.9 & -- & -- & -- & -- &  -- & -- & -- & -- \\
      % & T-L & 0.0 & -- & -- & -- & -- & -- & -- & -- & --\\
     % \hline
     % \hspace{-2mm}
     \textbf{(a) view hierarchy} & & & \\
     T + BT & 33.8 & 16.3 & 27.6 \\
     % & 0.0 & 0.0 & 4.5 & 6.5 & 9.5 & 9.5 & 23.3 & 22.1 & 27.0 \\
      T + BT + ID & 32.4 & 14.1 & 26.8 \\
       % 5.5 & 3.2 & 11.8 & 1.1 & 6.2 & 1.1 & 24.7 & 20.4 & 21.3  \\
     T + BT + ID + CLS & 27.3 & 15.2 & 34.3 \\
      % 11.0 & 10.2 & 7.4 & 5.7 & 2.3 & 9.3 & 17.0 & 18.9 & 19.3  \\
     T + Screen2Vec & 25.2 & 23.8 & \textbf{37.3} \\
      % 2.2 & 0.0 & 2.2 & 0.0 & 0.0 & 1.1 & 25.5 & 23.7 & 30.0 \\
      \hline
      \textbf{(b) app screen} & & & \\
      T + ResNet & 14.9 & 6.3 & 31.2\\
      % 0.0 & 0.0 & 0.0 & 11.3 & 0.0 & 4.4 & 3.3 & 14.8 & 23.9 \\
     T + Icons & 17.8 & 0.0 & 19.6 \\
      % 0.0 & 0.0 & 0.0 & 6.5 & 4.2 & 10.4 & 25.9 & 0.0 & 20.2 \\
      \hline
      \textbf{(c) best combo} & & & \\
      T + Screen2Vec + ResNet &\textbf{35.0} & \textbf{36.9} & 37.0\\
      % \hspace{-2mm}&\hspace{-.5mm} + ResNet & & & \\
      % 0.0 & 1.1 & 0.0 & 4.2 & 3.3 & 10.3 & 30.2 & 25.8 & 28.6 \\
      \hline
    \end{tabular}
    \caption{Task feasibility F1 score using a simple Multi-Layer Perceptron. We provide an ablation over input features and how features are aggregated over time.}% of the (a) view hierarchy and (b) image screen. The last row (c) uses the combination of best performing features.} %, \ie, we use the Screen2Vec and icon features for the view hierarchy and the screen, respectively.}
    \label{tab:feas}
    \vspace{-4mm}
\end{table} 
